TOI-5126: A hot super-Neptune and warm Neptune pair discovered by $\textit{TESS}$ and $\textit{CHEOPS}$

We present the confirmation of a hot super-Neptune with an exterior Neptune companion orbiting a bright (V = 10.1 mag) F-dwarf identified by the $\textit{Transiting Exoplanet Survey Satellite}$ ($\textit{TESS}$). The two planets, observed in sectors 45, 46 and 48 of the $\textit{TESS}$ extended mission, are $4.74^{+0.16}_{-0.14}$ $R_{\oplus}$ and $3.86^{+0.17}_{-0.16}$ $R_{\oplus}$ with $5.4588385^{+0.0000070}_{-0.0000072}$ d and $17.8999^{+0.0018}_{-0.0013}$ d orbital periods, respectively. We also obtained precise space based photometric follow-up of the system with ESAs $\textit{CHaracterising ExOplanets Satellite}$ ($\textit{CHEOPS}$) to constrain the radius and ephemeris of TOI-5126 b. TOI 5126 b is located in the "hot Neptune Desert" and is an ideal candidate for follow-up transmission spectroscopy due to its high predicted equilibrium temperature ($T_{eq} = 1442^{+46}_{-40}$ K) implying a cloud-free atmosphere. TOI-5126 c is a warm Neptune ($T_{eq}= 971^{+31}_{-27}$ K) also suitable for follow-up. Tentative transit timing variations (TTVs) have also been identified in analysis, suggesting the presence of at least one additional planet, however this signal may be caused by spot-crossing events, necessitating further precise photometric follow-up to confirm these signals.

==> authors.tex <==

%

\author[T.R. Fairnington et al.]{%
Tyler~R.~Fairnington%
\textsuperscript{\href{https://orcid.org/0000-0002-0692-7822}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{1}%
\thanks{Email: tyler.fairnington@gmail.com }
Emma Nabbie%
\textsuperscript{\href{https://orcid.org/0000-0003-0571-2245}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{1}
Chelsea~X.~Huang%
\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{1}
\thanks{ARC DECRA Fellow}
George Zhou%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{1}
\thanks{ARC DECRA Fellow}
Orion Foo%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
\newauthor
Sarah Millholland%
\textsuperscript{\href{https://orcid.org/0000-0003-3130-2282}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
Duncan Wright%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{1}
Alexandre~A.~Belinski%
\textsuperscript{\href{https://orcid.org/0000-0003-3469-0989}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{3}
Allyson Bieryla%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
David R. Ciardi %
\textsuperscript{\href{https://orcid.org/0000-0002-5741-3047}{\includegraphics[width=2.5mm]{orcid-ID.png}}}
,\textsuperscript{5}
\newauthor
Karen A.\ Collins%
\textsuperscript{\href{https://orcid.org/0000-0001-6588-9574}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
Kevin I.\ Collins%
\textsuperscript{\href{https://orcid.org/0000-0003-2781-3207}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{6}
Mark Everett%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{7}
Steve~B.~Howell%
\textsuperscript{\href{https://orcid.org/0000-0002-2532-2853}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{8}
Jack J. Lissauer%
\textsuperscript{\href{https://orcid.org/0000-0001-6513-1659}{\includegraphics[width=2.5mm]{orcid-ID.png}}}
,\textsuperscript{8}
\newauthor
Michael B. Lund%
\textsuperscript{\href{https://orcid.org/0000-0003-2527-1598}{\includegraphics[width=2.5mm]{orcid-ID.png}}}
,\textsuperscript{5}
Felipe Murgas%
\textsuperscript{\href{https://orcid.org/0000-0001-9087-1245}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{9,10}
Enric Palle%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{9,10}
Samuel N. Quinn%
\textsuperscript{\href{https://orcid.org/0000-0002-8964-8377}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
Howard M. Relles%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
\newauthor
Boris~S.~Safonov%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{3}
Richard P. Schwarz%
\textsuperscript{\href{https://orcid.org/0000-0001-8227-1020}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
Nicholas~J.~Scott%
\textsuperscript{\href{https://orcid.org/0000-0003-1038-9702}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{8}
%\newauthor
Gregor Srdoc%
%\textsuperscript{\href{https://orcid.org/0000-0003-0918-7484}%{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{12}
George Ricker
\textsuperscript{\href{https://orcid.org/0000-0003-2058-6662}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
\newauthor
Roland Vanderspek
\textsuperscript{\href{https://orcid.org/0000-0001-6763-6562}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
Sara Seager
\textsuperscript{\href{https://orcid.org/0000-0002-6892-6948}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{13,2,14}
David W. Latham
\textsuperscript{\href{https://orcid.org/0000-0001-9911-7388}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{4}
Joshua W. Winn
\textsuperscript{\href{https://orcid.org/0000-0002-4265-047X}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{15}\newauthor
Jon M. Jenkins
\textsuperscript{\href{https://orcid.org/0000-0002-4715-9460}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{8}
%Thomas~Barclay
%\textsuperscript{\href{https://orcid.org/0000-0001-7139-2724}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
%,\textsuperscript{16,17}
Luke~G.~Bouma
\textsuperscript{\href{https://orcid.org/0000-0002-0514-5538}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{16}\thanks{51 Pegasi b Fellow}
%John~P.~Doty
%\textsuperscript{\href{https://orcid.org/0000-0002-0514-5538}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
%,\textsuperscript{19}
Avi Shporer
%\textsuperscript{\href{https://orcid.org/0000-0002-0514-5538}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
Eric B. Ting 
\textsuperscript{\href{https://orcid.org/0000-0002-8219-9505}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{8}
Diana Dragomir
\textsuperscript{\href{https://orcid.org/0000-0003-2313-467X}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{17}
\newauthor
Michelle Kunimoto
%\textsuperscript{\href{https://orcid.org/0000-0002-8219-9505}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{2}
Nora L. Eisner
\textsuperscript{\href{https://orcid.org/ 0000-0002-0786-7307}{\includegraphics[width=2.5mm]{orcid-ID.png}}}%
,\textsuperscript{18, 15}
\\
\\
Affiliations are listed at the end of the paper
% (Author list is generated by script; will be updated to include new coauthors before submission)
}



